Response-Time-Optimized Distributed Cloud Resource Allocation

A current trend in networking and cloud computing is to provide compute resources over widely dispersed places exemplified by initiatives like Network Function Virtualisation. This paves the way for a widespread service deployment and can improve service quality; a nearby server can reduce the user-perceived response times. But always using the nearest server is a bad decision if that server is already highly utilized. This paper investigates the optimal assignment of users to widespread resources -- a convex capacitated facility location problem with integrated queuing systems. We determine the response times depending on the number of used resources. This enables service providers to balance between resource costs and the corresponding service quality. We also present a linear problem reformulation showing small optimality gaps and faster solving times; this speed-up enables a swift reaction to demand changes. Finally, we compare solutions by either considering or ignoring queuing systems and discuss the response time reduction by using the more complex model. Our investigations are backed by large-scale numerical evaluations.

==> documentProperties.tex <==
%
%
%
%
\RequirePackage[l2tabu, orthodox]{nag}

%
%
\newcommand{\ifdebug}[2]{ %
\ifthenelse{\isundefined{\mydebugmode}}{#2}{#1}
}

%
%
%
%
%

\usepackage{ifthen}

\usepackage{layouts}



%
%
%

\usepackage{graphicx}
\usepackage{caption}
%
\usepackage{subcaption}
\usepackage{wrapfig}
\usepackage{placeins}
\graphicspath{{./fig/}{./work/}}
\DeclareGraphicsExtensions{.pdf,.jpg,.jpeg,.png}
\usepackage{xcolor}


%
%


%
%

%
%
%
%
%



\usepackage{url}




%
%



%
%
%
%
%

\usepackage[utf8]{inputenc}
\usepackage[ngerman, english]{babel}
\hyphenation{op-tical net-works semi-conduc-tor brain-strom-ing in-di-vid-ual}


%
%



%
%

%
%
%
%
%

%
%
%


%
%
%
%
\usepackage{./style/tweaklist}
\renewcommand{\enumhook}{
	\setlength{\topsep}{0pt}  
	\setlength{\itemsep}{-0.6\baselineskip}
	\renewcommand{\labelenumi}{\alph{enumi})}}
	
	
%
\usepackage{paralist}

%
\renewcommand{\itemhook}{%
  \setlength{\topsep}{0pt}%
  \setlength{\itemsep}{-0.6\baselineskip}}
  
\renewcommand{\descripthook}{%
  \setlength{\topsep}{0pt}%
  \setlength{\itemsep}{0pt}}
  
  
  
%
%





%
%
%

\usepackage{textcomp}
\usepackage{amssymb, amsmath}
\allowdisplaybreaks %<- amsmath disable pagebreaks within equnarray environment, this reenables it

%
\usepackage{nicefrac}

%
%
%
%
%
%
%
%

\usepackage{siunitx}
\sisetup{ 
    per-mode = fraction,
    quotient-mode = fraction,
    fraction-function = \nicefrac, %
    decimalsymbol = {.}, %
    list-separator = {; },
    list-final-separator = {; },
    list-pair-separator = {; },
    list-units = single,  
    group-separator = {,} % enable ',' in 10,000
    %output-decimal-marker={,}% just uncomment if you want to use comma as the decimal marker!
}
\DeclareSIUnit\request{req.}
\DeclareSIUnit\req{\request}



%
%
%


\usepackage{listings}
\lstset{ %
  basicstyle=\footnotesize,           % the size of the fonts that are used for the code
  numbers=left,                   % where to put the line-numbers
  numberstyle=\tiny\color{gray},  % the style that is used for the line-numbers
  stepnumber=2,                   % the step between two line-numbers. If it's 1, each line 
                                  % will be numbered
  numbersep=5pt,                  % how far the line-numbers are from the code
  captionpos=b,
}

\usepackage{amsthm}
\theoremstyle{definition}
\newtheorem{theorem}{Theorem}
\newtheorem{definition}{Definition}
\newtheorem{lemma}{Lemma}
%

%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%


	

%
%
%

%
%


\ifdebug{
	\usepackage[draft, left, outer, marginal]{showlabels}
	\renewcommand{\showlabelfont}{ \small\sffamily\color{cyan} }
}{
    \usepackage[final]{showlabels}
}

\usepackage{newclude}
%
\usepackage{microtype}




%
%
%

%
%
%




%


%
%
%
%
%

%
%


%
%
%
%
%
%
%
\usepackage[sort,compress]{cleveref}
\crefname{table}{table}{tables}
\crefname{figure}{fig.}{fig.}   % <- IEEE specialiality
\crefname{section}{section}{sections}
\crefname{chapter}{chapter}{chapters}
\crefname{lstlisting}{listing}{listings}
\crefname{requestthm}{request}{requests}
%
\crefname{equation}{}{}
\crefformat{equation}{(#2#1#3)} %#1#3} %##1##3}
\newcommand{\crefrangeconjunction}{--}
\crefformat{footnote}{#2\footnotemark[#1]#3} % this allow referencing a already referenced footnote with a label
\newcommand{\Coref}[1]{Constraint~\eqref{#1}}

\renewcommand{\figurename}{Fig.}  % <- IEEE specialiality
   
 
%
%
%
%
   
\usepackage{setspace}
   
%
%
%

\ifdebug{
	\usepackage[inline,draft,index,multiuser,marginclue]{fixme}
	\fxsetup{theme=color}
}{
	\usepackage[final, multiuser]{fixme}
}


\FXRegisterAuthor{mk}{emk}{MK} % Matthias 
\FXRegisterAuthor{hk}{ehk}{HK} % HK
%
%
%
\newcommand{\fmhkn}[1]{\hkwarning{#1}}

%
%
%

%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
\usepackage{etoolbox}
\usepackage{comment}

%
%
%
%
%
%
%
%
%
%
%
%
%
%
     
\ifdefmacro\extendedversion{
    \ifdefstring\extendedversion{draft}{
        % extendedversion == draft
        \newcommand{\ifextended}[2][]{ %
            \bgroup\color{black!80} [EXT]~#2~%
            \ifstrempty{#1}{}{[NOEXT]~#1~}%
            \egroup}
               
        \newenvironment{inextended}[0] { %begin
                \bgroup \color{black!80}[EXT]~%        
            }{ %
                \egroup}
            
        \newenvironment{notinextended}[0] { %begin
                \bgroup \color{black!80}[NOEXT]~%        
            }{ %
                \egroup}
                               
    }{
    
        % extendedversion != draft
        \newcommand{\ifextended}[2][]{ %
            \bgroup #2 \egroup}

        \excludecomment{notinextended}
        
        \newenvironment{inextended}[0] { %begin
             \bgroup%
            }{ %
              \egroup}
    
    }

        
}{
    % not extendedversion 

    \newcommand{\ifextended}[2][]{ %
        \bgroup #1 \egroup}


    \excludecomment{inextended}
    
    \newenvironment{notinextended}[0] { %begin
            \bgroup%
        }{ %
            \egroup}

}


 
    
 %%%% CUSTOM COMMAND %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 %
    

\DeclareMathOperator*{\argmin}{arg\!min}
\DeclareMathOperator*{\dom}{dom}

\usepackage{xspace}

\renewcommand{\emph}{\textit}
\newcommand{\etal}[0]{~et\,al.}
\newcommand{\etalcite}[1]{~et\,al.~\cite{#1}}

\newcommand\eg{e.g.\@\xspace}
\newcommand\cf{c.f.\@\xspace}
\newcommand\vs{vs.\@\xspace}

%
\newcommand{\lcf}{l_{cf}}
\newcommand{\xcf}{x_{cf}}
\newcommand{\zfs}{z_{fs}}
\newcommand{\Rn}{\mathbf{R}^n}
\newcommand{\Rnm}{\mathbf{R}^{n \times m}}
\newcommand{\Rp}{\mathbf{R}_{\geq0}}
\newcommand{\Zp}{\mathbf{Z}_{\geq0}}
\newcommand{\Tamu}{T_{\mu_f} }
\newcommand{\sums}{\sum_s}
\newcommand{\sumf}{\sum_f}
\newcommand{\sumc}{\sum_c}
\newcommand{\qmmone}{$\rm{M}/\rm{M}/\rm{1}$ }

\newcommand{\optP}{\mathsf{P}}
\newcommand{\optQP}{\mathsf{QP}}
\newcommand{\optPQP}{\mathsf{PQP}}
\newcommand{\optQPa}{\widetilde{\mathsf{QP}}}
\newcommand{\funcT}{\mathsf{T}_\mu}
\newcommand{\funcTa}{\tilde{\mathsf{T}}_\mu}

\newcommand{\QFLP}{\mathsf{QF}_T }
\newcommand{\QFLPa}{\mathsf{\widetilde{QF}}_T }
\newcommand{\mQFLP}{\mathsf{mQF}_T }
\newcommand{\mQFLPa}{\mathsf{m\widetilde{QF}}_T}
\newcommand{\RT}{\emph{response time} }
\newcommand{\RTT}{\emph{round trip time} }
\newcommand{\PD}{\emph{processing time} }
\newcommand{\PDfunc}{T_{\mu_f}(\cdot)}
\newcommand{\PDfuncl}{T_{\mu_f}(\lambda')}
\newcommand{\unitreqs}{~\nicefrac{\unit{req}}{\unit{s}}}
\newcommand{\unitreqms}{~\nicefrac{\unit{req}}{\unit{ms}}}

%
%

%


%
%







